Cybercosm: New Foundations for a Converged Science Data Ecosystem

Scientific communities naturally tend to organize around data ecosystems created by the combination of their observational devices, their data repositories, and the workflows essential to carry their research from observation to discovery. However, these legacy data ecosystems are now breaking down under the pressure of the exponential growth in the volume and velocity of these workflows, which are further complicated by the need to integrate the highly data intensive methods of the Artificial Intelligence revolution. Enabling ground breaking science that makes full use of this new, data saturated research environment will require distributed systems that support dramatically improved resource sharing, workflow portability and composability, and data ecosystem convergence. The Cybercosm vision presented in this white paper describes a radically different approach to the architecture of distributed systems for data-intensive science and its application workflows. As opposed to traditional models that restrict interoperability by hiving off storage, networking, and computing resources in separate technology silos, Cybercosm defines a minimally sufficient hypervisor as a spanning layer for its data plane that virtualizes and converges the local resources of the system's nodes in a fully interoperable manner. By building on a common, universal interface into which the problems that infect today's data-intensive workflows can be decomposed and attacked, Cybercosm aims to support scalable, portable and composable workflows that span and merge the distributed data ecosystems that characterize leading edge research communities today.

==> proposal-summary.tex <==
%!TEX root = main.tex

% \begin{center}
% \textbf{\projectname: New Foundations for a Converged Science Data Ecosystem}
% \end{center}

% \vspace{10pt}

\pp{Overview} 
% Scientific communities have traditionally used a workflow paradigm in which data is repeatedly put into and taken out of technology silos for computing, networking, and storage. 
Scientific communities naturally tend to organize around data ecosystems created by the combination of their observational devices, their data repositories, and the workflows essential to carry their research from observation to discovery. However, these legacy data ecosystems are now breaking down under the pressure of exponential growth in data from highly data intensive methods introduced by the sea change in Artificial Intelligence (AI). A revolutionary ecosystem that enables science in this new era will require distributed systems that support dramatically improved resource sharing, workflow portability and composability, reproducibility, and data ecosystem convergence. In the Cybercosm Center for Converged Data Ecosystems, the PIs will articulate, catalyze, and carry out the fundamental research agenda needed to unify, and thereby revolutionize, the foundations on which tomorrow’s data ecosystems are built. 
% But the legacy workflow paradigm, in which data is repeatedly put into and taken out of traditional technology silos for computing, networking, and storage, is breaking down under the pressure of the exponential growth in the volume and velocity of these workflows and the need to integrate the highly data intensive methods of the Artificial Intelligence (AI) revolution. Filling this growing chasm will require distributed systems that support dramatically improved resource sharing, workflow portability and composability, and data ecosystem convergence. 
% Building on a radically different approach to distributed system architecture, the goal of the \projectname Center for Converged Data Ecosystems is to catalyze the fundamental research agenda needed to revolutionize the foundations on which tomorrow’s dramatically more interoperable data ecosystems will be built. 
The PIs will build a transformative ecosystem in \projectname by: 1) Collaborating with a wide range of application partners to drive innovation in the design of core services; 2) Defining an experimental system that can be readily deployed to support the collaborating communities; 3) Assembling a leadership team from the University of Tennessee - Knoxville, Georgia Institute of Technology, Indiana University, the University of California - San Diego, and Vanderbilt University that can draw together and coordinate a diverse and rapidly growing research community; and 4) Inspiring students and broadening participation over the life of the project and beyond.

%Scientists organize their research around data, but they have to deal with legacy workflow paradigms in which data is repeatedly put into and taken out of traditional technology silos for computing, networking, and storage/buffering. These legacy data workflows are breaking down by the volume of data, the exponentially growing velocity of data production, and the novel integration of Artificial Intelligence (AI) and Machine Learning (ML) methods.

%The goal of the Cybercosm Center for Converged Data Ecosystems is to articulate, catalyze, and help to carry out the fundamental research agenda needed to unify, and thereby revolutionize, the foundations on which tomorrow’s dramatically more interoperable data ecosystems will be built. Cybercosm will open up a transformative path forward both for CISE research and for cyberinfrastructure generally. This project builds upon the observation that data are collected as a set of buffers and computations as operations on the buffers. We leverage the principle that buffers can be implemented on existing technologies such as storage, networking, and architectures with various sizes, properties, and levels of abstractions, but we also propose new CI for more effective processing buffers in the modern era of data generated at the edge. By doing so we make buffers first class citizen in modern data ecosystems. Our principled approach for achieving scalability builds on spanning layers that form the ``waist'' of iconic ``hourglass'' system designs and exposes a common interface to generic buffers and operations performed in situ, with the buffer as the unit of service. Cybercosm will create a new foundation for distributed systems that facilitates resource sharing, workflow composability, and interoperable convergence among the data ecosystems of diverse scientific communities.

%\pp{Keywords} High-performance Computing; Federation of Distributed Resources; Cyberinfrastructures; Data Ecosystems; Layered and Resilient Systems

\pp{Intellectual Merit} Cybercosm will define a visionary research agenda and its revolutionary experimental system by rethinking the architecture of data-intensive science application workflows. It will disrupt the current siloed effects and restricted interoperability among scientific discoveries typical of the HPC-center models. The \projectname architecture will define scalable, portable, and composable workflows that span and merge data ecosystems by building on the transvisor service, a minimally sufficient hypervisor. The transvisor serves as a spanning layer for \projectname's ``data plane'' by providing a converged virtualization of the local resources of its distributed nodes. Cybercosm's design will build on an observation, a principle, and a strategy. The observation reveals a novel understanding of data as buffers, which become the essential building blocks of all digital systems because they are required for state management and programmable control. Thus, the primitive operations on buffers in \projectname's ``data plane'' construct the familiar abstractions of process, file, and flow as ``control plane'' services. The principle links the scalability of service specifications and the degree to which they are logically weak, simple, general, and resource limited. The PIs call this the deployment scalability tradeoff principle; it dramatically affects the potential for widespread adoption and use of service specifications. The PIs will combine this observation and this principle to implement \projectname's new  strategy for maximizing the leverage of participants and adopters while minimizing their risks. Ultimately, \projectname will fill in the ``missing middle'' of data ecosystem convergence by creating a type of converged distributed system that is purpose-built for deployment scalability. 

%The Cybercosm architecture will support scalable, portable and composable workflows that span and merge data ecosystems by building on a universal service---the transvisor service--into which all that problems that infect today's data intensive workflows can be decomposed and attacked. The transvisor mechanism is a minimally sufficient hypervisor that provides a converged virtualization of the local resources (i.e. storage, processing, and transfer) of the individual nodes of a distributed system. 

%Cybercosm defines a visionary research agenda and its revolutionary experimental system by rethinking the architecture of data-intensive science application workflows and disrupting the current siloed effects and restricted interoperability among scientific discoveries typical of technology and service stacks used by the HPC-center model. The revolutionary components of this project are: the transvisor service that is both non-localized and distributed, so no topological constraints exist; the resource availability without reservation, so no temporal constraints exist; the architectural abstractions,so no architectural constraints exist; and the unmetered and unbounded aggregation and federation of resources, so significantly reduced resource constraints are in place. The Cybercosm Center is led by its outstanding group of PIs, each bringing different, complementary areas of expertise to the project.

\pp{Broader Impacts} By dissolving the walls separating traditional technology silos, \projectname will have a significant economic, social, and scientific impact on next generation cyberinfrastructure. Rather than each field re-implementing common functionality, \projectname R\&D communities can produce common control plane tools and libraries to provide such functions as well as create entirely new services based on novel abstractions that cross legacy silo boundaries. \projectname's success will create a scalable, interoperable, compute-enabled system of data ecosystems, incorporating NSF-funded facilities like FABRIC and XSEDE, 
%that is essential for the development of technologies like open and affordable content distribution networks and composable wide-area data-intensive workflows. Cybercosm 
that will offer an unprecedented environment for supporting research and experimentation on new services by the CISE and CI research communities. The Broader Participation Plan will engage underrepresented communities by recruiting faculty from community colleges and predominantly undergraduate institutions in three states (i.e., Tennessee, Georgia, and Indiana) in transforming the experience of application users into training and educational materials. These materials will allow participating faculty to engage a diverse population of students in the STEM pipeline in research-discovery activities (including students from the Consortium of Historically Black Colleges in Atlanta and surrounding areas through the support of the Big Data South Hub). 
